Observation of unconventional spin polarization induced spin orbit torque in L1$_2$-ordered antiferromagnetic Mn$_3$Pt thin films

Non-collinear antiferromagnets exhibits richer magneto-transport properties due to the topologically nontrivial spin structure they possess compared to conventional nonmagnetic materials, which allows us to manipulate the charge-spin conversion more freely by taking advantage of the chirality. In this work, we explore the unconventional spin orbit torque of L1$_2$-ordered Mn$_3$Pt with a triangular spin structure. We observed an unconventional spin orbit torque along the $\mathbf{x}$-direction for the (001)-oriented L1$_2$ Mn$_3$Pt, and found that it has a unique sign reversal behavior relative to the crystalline orientation. This generation of unconventional spin orbit torque for L1$_2$-ordered Mn$_3$Pt can be interpreted as stemming from the magnetic spin Hall effect. This report help clarify the correlation between the topologically nontrivial spin structure and charge-spin conversion in non-collinear antiferromagnets.

==> tex/01_model.tex <==
\section{TEST}

